Quantum Computation of Frequency-Domain Molecular Response Properties Using a Three-Qubit iToffoli Gate

The quantum computation of molecular response properties on near-term quantum hardware is a topic of significant interest. While computing time-domain response properties is in principle straightforward due to the natural ability of quantum computers to simulate unitary time evolution, circuit depth limitations restrict the maximum time that can be simulated and hence the extraction of frequency-domain properties. Computing properties directly in the frequency domain is therefore desirable, but the circuits require large depth when the typical hardware gate set consisting of single- and two-qubit gates is used. Here, we report the experimental quantum computation of the response properties of diatomic molecules directly in the frequency domain using a three-qubit iToffoli gate, enabling a reduction in circuit depth by a factor of two. We show that the molecular properties obtained with the iToffoli gate exhibit comparable or better agreement with theory than those obtained with the native CZ gates. Our work is among the first demonstrations of the practical usage of a native multi-qubit gate in quantum simulation, with diverse potential applications to the simulation of quantum many-body systems on near-term digital quantum computers.

==> gate_cal_figure/circuit_drawer.tex <==
\begin{quantikz}[row sep={0.8cm,between origins},column sep={0.4cm}]
    \lstick{{\fontfamily{phv}\selectfont Q$_{0}$}} & \gate{X_{\pi}} & \gate[wires=4]{U_{i\text{\fontfamily{phv}\selectfont TOF}}} & \qw & \qw & \meter{} \\
    \lstick{{\fontfamily{phv}\selectfont Q$_{1}$}} & \qw & & \qw & \qw & \meter{} \\
    \lstick{{\fontfamily{phv}\selectfont Q$_{2}$}} & \gate{{\color{firebrick} X_{\pi}}\ /\ {\color{slateblue} I}} & & \qw & \qw & \meter{} \\
    \lstick{{\fontfamily{phv}\selectfont Q$_{3}$}} & \gate{X_{\pi/2}} & & \gate{Z_{\phi}} & \gate{X_{\pi/2}} & \meter{}
\end{quantikz}

\newpage

\begin{quantikz}[align equals at=2.5, row sep={0.8cm,between origins},column sep={0.4cm}]
    \qw & \octrl{1} & \qw \\
    \qw & \gate{iX} & \qw \\
    \qw & \octrl{-1} & \qw \\
    \qw & \gate{I} & \qw
\end{quantikz}=\begin{quantikz}[align equals at=2.5, row sep={0.8cm,between origins},column sep={0.4cm}]
    \qw & \gate[wires=4]{U_{i\text{\fontfamily{phv}\selectfont TOF}}} & \qw & \qw \\
    \qw & & \qw & \qw \\
    \qw & & \ctrl{1} & \qw \\
    \qw & & \gate{Z_{\varphi}} & \qw
\end{quantikz}

==> gate_cal_figure/gatecal.tex <==
This work employs the recently developed $C-iX-C$ iToffoli gate \cite{kim_2022}. Since the gate acts on a three qubit subset of the full four qubit subsystem we need to understand and correct the spectator error on the fourth qubit. For concreteness we label qubits $Q_{i}$ for $i=0,\dots,3$ with the iToffoli acting on $Q_{0}$, $Q_{1}$, and $Q_{2}$ with $Q_{3}$ as spectator and denote states in the form $\ket{Q_{0}Q_{1}Q_{2}Q_{3}}$. We run a simple circuit where we prepare the system in either $\ket{100+}$ or $\ket{101+}$ ($\ket{+}=(\ket{0}+\ket{1})/\sqrt{2}$) and apply the iToffoli gate to determine the $Z$ rotation on $Q_{3}$ conditional on the state of its nearest neighbor, $Q_{2}$ (see Fig.~ for circuit diagram). We observe an unwanted conditional phase interaction between $Q_{2}$ and $Q_{3}$ with conditional phase, $\phi = 0.844$ (see Fig.~). This interaction results from the conditional Stark shift between $Q_{2}$ and $Q_{3}$ when a strong off resonant drive is applied to $Q_{2}$ at the frequency of $Q_{1}$ to implement the iToffoli gate \cite{mitchell_2021}. We can use the same effect to undo the conditional phase by applying simultaneous off-resonant drives to $Q_{2}$ and $Q_{3}$ for a $120~\text{ns}$ period following the iToffoli drive sequence (see Fig.~ for the pulse sequence and characterization of the conditional rotation with the cancellation applied). We benchmark the resulting gate implementation using Cycle Benchmarking \cite{erhard_2019}. With this correction, we measure a gate fidelity of $97.5\%$ when isolated to the cycle involving qubits that participate in the iToffoli gate, and a small reduction to $96.1\%$ when including the idling spectator qubit.

In order to mitigate errors and improve algorithm performance we apply a modified version of Randomized Compiling (RC) \cite{hashim_2021_randomized, wallman_2016} to the circuits used to compute the observables in the main text. A broad native entangling gate set is used, consistent of both Clifford gates (CZ) and non-Clifford gates (CS$^{\dagger}$, CS, iToffoli). RC is typically used with hard cycles of $n$-qubit Cliffords in which case the twirling group $\mathcal{T}$ is chosen to be the group of tensor products of $n$ single qubit Paulis. By the definition of Clifford gates, for any Clifford $C$ and twirling gate $T \in \mathcal{T}$ there is some $T^{c} \in \mathcal{T}$ such that $C=TCT^{c}$. RC applied to hard cycles of Clifford gates, $C_{k}$ then proceeds by choosing some $T_{k}$ for each hard cycle $k$, letting $C_{k} \rightarrow T_{k}C_{k}T_{k}^{c}$ and compiling the single qubit Paulis $T_{k}$ and $T_{k}^{c}$ into the easy cycles of single qubit gates before and after, respectively, the Clifford cycle $C_{k}$. 

In order to generalize the method to the non-Clifford gates employed in this work we first find the subsets $\mathcal{T}_{X} \subset \mathcal{T}$ for $X=\mathrm{CS},\mathrm{CS}^{\dagger},\mathrm{iToffoli}$ where for all $T \in \mathcal{T}_{X}$ there is some $T^{c} \in \mathcal{T}_{X}$ such that $X=TXT^{c}$. Then RC proceeds in the same way as above except the twirling gates for hard cycles consisting of gate $X$ are simply chosen from the subset $\mathcal{T}_{X}$ of Pauli strings that stabilize gate $X$. Both the CS and CS$^{\dagger}$ are stabilized by 4 of the possible 16 two-qubit Pauli strings and the iToffoli is stabilized by 8 of the possible 64 three-qubit Pauli strings. For all these non-Clifford gates the twirling and inversion gate are the same, $T=T^{c}$. Results ``with RC'' in the main text involve averaging the experimental bitstring output distributions over 100 equivalent circuit randomizations according to the process outlined here, with each circuit measured for 500 shots. These are compared to results ``without RC'' in which the bare circuit is measured for 50000 shots (such that the total number of shots is maintained between the two implementations).

All error processes can be described by a superoperator $\mathcal{E}$ acting on the system density matrix $\rho$. Written in the $n$-qubit Pauli basis this error process matrix is referred to as a Pauli Transfer Matrix (PTM) with diagonal elements giving the rate of stochastic Pauli (incoherent) errors and off-diagonal elements characterizing the unitary (coherent) errors. As discussed in \cite{hashim_2021_randomized, wallman_2016}, applying RC tailors coherent errors into stochastic Pauli noise, which suppresses the off-diagonal elements of the PTM. This holds for the PTM describing errors during the CZ cycles, since these undergo perfect Pauli twirling. However, in the case of the non-Clifford gate cycles, the twirling is imperfect (since we only twirl over a subset of the $n$-qubit Pauli strings). As a result, some, but not all, of the off-diagonal elements in the corresponding PTMs are suppressed. In other words, not all coherent errors are tailored to stochastic Pauli noise, This imperfect noise tailoring is the main limitation of our approach to generalizing RC to non-Clifford gates. 

==> scratch <==
% and points to how multi-controlled gates and density matrix purity constraints can be utilized to improve LCU-based algorithms.


% exemplified by the iToffoli gate
% Error mitigation techniques involving randomized compiling and McWeeney purification are shown to significantly improve the raw experimental results. 


% We compute spectral functions and density-density response functions of diatomic molecules NaH and KH, where t

% determining response properties directly in the frequency domain has been challenging. In this work, we experimentally demrate a recently proposed quantum algorithm based on linear combination of unitaries (LCU) to compute frequency-domain response properties of molecules by employing a high-fidelity three-qubit iToffoli gate.

%its potential advantages to two-qubit gates in implementing quantum algorithms that naturally involve multi-controlled gates.

%Our work demates that multi-controlled gates exemplified by the iToffoli gate are advantageous to two-qubit gates in quantum simulation and can be considered a native gate component in future quantum algorithm design.

%*****there are a lot of papers that should be added to the discussion here. e.g. finite temperature, work of kemper/freericks, simon benjamin, etc


% As quantum advantages in random sampling have been established on quantum hardware \cite{google_2019,wu_2021}, the next frontier of quantum computing is to experimentally demonstrate quantum advantages in tasks of practical interest especially in simulating physical systems \cite{daley_2022}. }

%{\color{cyan} and disc....omalley 2016 and cite some recent ones, go over types of calculations, etc. aim for 3-4 more sentences.}

%to study neutron scattering \cite{chiesa_2019}, magnon spectra \cite{francis_2020}, and finite-temperature dynamics of spin systems \cite{sun_2021}. 

%However, due to Trotterization of the time-evolution operator \cite{hatano_2005}, these time-domain quantum algorithms are generally restricted to insufficient time duration owing to circuit depth limitations. 


% Much research effort has been devoted to computing time-domain response properties of many-body physical systems on quantum computers due to the natural ability of quantum devices to simulate the time evolution of quantum systems \cite{feynman_1982,lloyd_1996}. 
%Thanks to advancement in superconducting circuit-based quantum processors in the past two decades \cite{krantz_2019,kjaergaard_2020,blais_2021}, 

%Our work establishes the practical usage of multi-qubit gates in quantum simulation, with diverse potential applications in the simulation of quantum many-body systems on near-term hardware.
% Our work explores a new path of determining frequency-domain molecular response properties on near-term quantum hardware by utilizing native high-fidelity three-qubit gates to implement LCU-based quantum simulation protocols.


% \begin{table*}
% \centering
% \begin{tabular}{|O|C|C|}
% \hline
% \multirow{2}{*}{Orbitals} & \multicolumn{3}{c|}{iToffoli circuits} & \multicolumn{3}{c|}{CZ circuits} \\ \cline{2-7}
%  & Depth & \# CZ/CS/CS$^\dagger$ & \# iToffoli & Depth & \# CZ/CS/CS$^{\dagger}$ & \# iToffoli  \\
% \hline
% 0$\uparrow$, 0$\downarrow$ & 54 & 22 & 3 & 87 & 37 & 0 \\
% 0$\uparrow$, 1$\uparrow$   & 51 & 20 & 3 & 83 & 36 & 0 \\
% 0$\uparrow$, 1$\downarrow$ & 35 & 14 & 2 & 59 & 26 & 0 \\
% 0$\downarrow$, 1$\uparrow$ & 58 & 22 & 4 & 107 & 46 & 0 \\
% 0$\downarrow$, 1$\downarrow$ & 51 & 20 & 3 & 83 & 36 & 0 \\
% 1$\uparrow$, 1$\downarrow$ & 47 & 18 & 3 & 80 & 34 & 0\\
% \hline
% \end{tabular}
% \caption{Circuit depths and multi-qubit gate counts of four-qubit response function circuits after applying all transpilation techniques (see Methods). Depths of the circuits with CZ decompositions are 1.5 to 2 times of those with iToffoli decomposition, and the number of two-qubit gate counts almost double those of the iToffoli circuits.}
% \label{tab:circuit_statistics}
% \end{table*}

% The number of iToffoli gates, which corresponds to the number of CCZ gates in the original circuits, range from two to four, with the circuit with two iToffoli gates being the shortest and the circuit with four iToffoli gates being the deepest. Because each CCZ gate requires 6 CZ gates in the decomposition, the number of two-qubit gates nearly double that of the two-qubit gates in iToffoli decomposition. The circuit depths of the CZ decomposition are also 1.5 to 2 times of that of the circuits with iToffoli decomposition.

with the major fidelity decreases occurring near the locations of the iToffoli gates

%{\color{magenta} ****I think we should consider a reorder of the figures. It doesn't seem to flow well to talk about a quantity for a long time and then only show it at the end. I suggest the order as Fig 6, 5, 4. We can talk about it The logic would be, show the results, then go into more investigation about the reason for the comparable or improved performance in terms of fidelity, and then the main result is better fidelity with a multiqubit gate circuit.}

% ***we should talk about this para

% The matrices are labeled such that the elements correspond to the circuit indexed by the row and column indices, with the upper (lower) diagonal part corresponding to the ancilla sector $(a_0, a_1) = (1, 0)$ ($(a_0, a_1) = (1, 1)$). Figure \ref{fig:fidelity_matrix} shows results

%For example in Fig.~\ref{fig:chi00_rc}, in the iToffoli decomposition the peak height deviations are 11.8\% and 24.0\%, while in the CZ decomposition the peak height deviations are 34.8\% and 4.8\%. 
%**********we will likely be asked to provide quantitative justification for this statement

%the deviations of the two peaks in Fig.~\ref{fig:chi00_norc} are 6.1\% and 26.6\%, whereas the CZ decomposition yields a peak that has more than twice the height of the exact peak at $\pm 1.4$ eV, and fails to produce a peak at $\pm24$ eV.

% Compared to previous experimental demonstrations of quantum algorithms to compute response properties on quantum hardware \cite{huang_2022}, we showed that a non-variational algorithm is able to yield response properties directly in the frequency domain with reduced quantum resources using 

% achieve great accuracy with quantum resource reduction, error mitigation and especially a native implementation of a high-fidelity multi-qubit gate.

% ********pls make this part more quantitative e.g. limited extent, significant improvement, and so on can be quantified

%****numbers?

%Compared to previous studies on applying both RC and McWeeney purification to the quantum algorithm, 
%but the use of RC and especially in combination with McWeeney purification in quantum computation has been explored only recently \cite{ville_2022}. In Ref.~\cite{ville_2022}, the authors find that RC and purification improve the results separately, with the best performance achieved when both are applied. 

%uclear structure \cite{siwach_2022} and non-Hermitian dynamics \cite{wen_2019}
%due to low fidelity in early implementations of three-qubit gates \cite{mariantoni_2011,fedorov_2012,reed_2012} which are prone to decoherence and leakage. More recent three-qubit gates \cite{kim_2022,hill_2021,galda_2021} increase in fidelities and can be applied on scalable architectures. }
% As such native multi-qubit gates achieve fidelities comparable to those of single- and two-qubit gates and become available in a wider range of architectures, our work paves the way for using multi-qubit gates as native gate components in future quantum algorithm design and implementation. }

%Our results provide insight into demonstrating general LCU algorithms on quantum hardware with multi-qubit gates.

% {\color{magenta} **I think you could make a marginally stronger claim here ***I would somehow arrange this to end with the strong claim regarding multi-qubit gates} 

%\begin{figure}[h]
%\centering
%\includegraphics[width=0.9\textwidth]{fig2_ccz_decomposition.png}
%\caption{Decomposition of the CCZ gates in the algorithm. (a) Decomposition using the three-qubit iToffoli gate. (b) Decompositing using CZ gates.}
%\label{fig:ccz_decomposition}
%\end{figure}

% In the quantum algorithm in this work, the creation and annihilation operators map the original $N$-electron ($N = 2$) states to $(N\pm1)$-electron states, shown in Table I.

% \begin{table}[H]
% \normalsize
% \centering
% \begin{tabular}{c|c|c}
% \hline\hline
% & $\uparrow$ & $\downarrow$ \\
% \hline
% ($N$+1) electrons & 0111, 1101 & 1011, 1110\\
% \hline
% ($N$-1) electrons & 0001, 0100 & 0010, 1000\\
% \hline\hline
% \end{tabular}
% \caption{($N\pm$1)-electron qubit states}
% \end{table}

% We can characterize the eight $(N\pm1)$-electron states with by the expectation values of $ZIZI$ and $IZIZ$ as well. Note that $(N+1)$-electron spin-up states and $(N-1)$-electron spin-down states have the expectation values
% \begin{align}
% \langle IZIZ\rangle = +1, \quad \langle ZIZI\rangle = -1
% \end{align}
% and are produced by acting $\hat{a}_{m\uparrow}^{(\dagger)}$ on the ground state. On the other hand, the $(N+1)$-electron spin-down states and $(N-1)$-electron spin-up states have the expectation values
% \begin{align}
% \langle IZIZ\rangle = -1, \quad \langle ZIZI\rangle = +1
% \end{align}
% and are obtained from acting $\hat{a}_{m\downarrow}^{(\dagger)}$ on the ground state.

% \begin{table}[H]
% \normalsize
% \centering
% \begin{tabular}{c|c|c}
% \hline\hline
% & $\uparrow$ & $\downarrow$ \\
% \hline
% ($N+1$) electrons & 01, 11 & 10, 11\\
% \hline
% ($N-1$) electrons & 00, 01 & 00, 10\\
% \hline\hline
% \end{tabular}
% \caption{($N\pm$1)-electron qubit states after $\mathbb{Z}_2$ symmetry transformations.}
% \end{table}

%\begin{figure}[h]
%\centering{\includegraphics[width=0.48\textwidth]{fig2_itoffoli_vs_cz.png}}
%\caption{Spectral function and density-density response function by comparing iToffoli decomposition and CZ decomposition. (a)(b) Spectral function of NaH and KH, calculated from the diagonal elements of the Green's function. (c)(d) Imaginary part of the density-density response function between HOMO and HOMO of NaH and KH. (e)(f) Imaginary part of the density-density response function between HOMO and LUMO of NaH and KH. Not much discrepancy between experimental and exact results can be observed in the spectral function because they only involve shallow three-qubit circuits. In both $\chi_{00}$ and $\chi_{11}$, the iToffoli decomposition appears to yield better agreement with the exact results by getting the correct signs and sometimes the amplitudes of the peaks, whereas the CZ decomopsition gave the wrong signs on the side peaks in both observables.}
%\end{figure}

\onecolumngrid

\clearpage


%\begin{figure}[h]
%\centering{
%\includegraphics[width=0.95\textwidth]{fig3_error_analysis.png}
%}
%\caption{Error analysis of density-density response functions by examining system-qubit reduced density matrices and ancilla bitstring probabilities. (a) Purities of the experimental system-qubit reduced density matrices. The diagonal elements correspond to the diagonal circuits,  the upper triangular elements correspond to $p$ and lower triangular elements correspond to $m$ elements. (b) Fidelities between the experimental reduced density matrices and the exact reduced density matrices on the system qubits. The values in parentheses are the fidelities after purification. (c) Traces of the experimental reduced density matrices, which correspond to the ancilla bistring probabilities. The exact traces are shown in the parentheses. Colors of the tiles reflect the difference between the experimental trace and the exact trace. (d)(e) Observables without postprocessing (raw), with density-matrix purification (purified) and with both McWeeney purification and trace correction (purified + trace-corrected). Trace correction does not necessarily improve the experimental results, indicating that the fidelities after purification are still not high enough.}
%\label{fig:response_function}
%\end{figure}

\begin{table}[b]
\centering
\begin{tabular}{|Q|O|C|C|}
\hline
\multirow{2}{*}{Quantity} & \multirow{2}{*}{Orbitals} & \multicolumn{3}{c|}{iToffoli circuits} & \multicolumn{3}{c|}{CZ circuits} \\ \cline{3-8}
 &  & Depth & \# CZ/CS/CS$^\dagger$ & \# iToffoli & Depth & \# CZ/CS/CS$^{\dagger}$ & \# iToffoli  \\
\hline
%\multirow{3}{*}{\shortstack{Green's\\ function}} 
%    & 0$\uparrow$ & 8 & 3 &          0 & 8 & 3 & 0\\
%    & 1$\uparrow$ & 16 & 7 & 0 & 16 & 7 & 0\\
\shortstack{Green's\\ function}
    & 0$\uparrow$, 1$\uparrow$ & 49 & 22 & 3 & 78 & 33 & 0\\ \hline
%\multirow{10}{*}{\shortstack{Response\\ function}} & 0$\uparrow$ & 13 & 6 & 0 & 13 & 6 & 0\\
%    & 0$\downarrow$ & 18 & 7 & 0 & 18 & 7 & 0 \\
%    & 1$\uparrow$ & 15 & 6 & 0 & 15 & 6 & 0 \\
%    & 1$\downarrow$ & 8 & 3 & 0 & 8 & 3 & 0  \\
\multirow{6}{*}{\shortstack{Response\\ function}}
    & 0$\uparrow$, 0$\downarrow$ & 54 & 22 & 3 & 87 & 37 & 0 \\
    & 0$\uparrow$, 1$\uparrow$   & 51 & 20 & 3 & 83 & 36 & 0 \\
    & 0$\uparrow$, 1$\downarrow$ & 35 & 14 & 2 & 59 & 26 & 0 \\
    & 0$\downarrow$, 1$\uparrow$ & 58 & 22 & 4 & 107 & 46 & 0 \\
    & 0$\downarrow$, 1$\downarrow$ & 51 & 20 & 3 & 83 & 36 & 0 \\
    & 1$\uparrow$, 1$\downarrow$ & 47 & 18 & 3 & 80 & 34 & 0\\
\hline
\end{tabular}
\caption{Circuit depths and multi-qubit gate counts of all the experimental circuits. Only up-spin orbitals are involved in calculating the Green's function circuits due to spin symmetry. The circuits involving only one orbital (e.g. 0$\uparrow$) are the three-qubit circuits without the iToffoli gates, and the circuits involving two orbitals (e.g. $0\uparrow, 0\downarrow$) are the four-qubit circuits with the iToffoli gates.}
\label{tab:circuit_stats}
\end{table}


 %(\textbf{E} to \textbf{F}) Effect of trace correction in addition to McWeeney purification. (E) $\Im\,\chi_{01}$ without RC. (F) $\Im\,\chi_{01}$ with RC. Without RC trace correction does not improve the experimental results since fidelities on the system-qubit density matrices are not high enough. With RC the fidelities of the system-qubit density matrices are over 98\%, and hence trace correction yields almost exact results.
